An Intelligent Agentic System for Complex Image Restoration Problems

Real-world image restoration (IR) is inherently complex and often requires combining multiple specialized models to address diverse degradations. Inspired by human problem-solving, we propose AgenticIR, an agentic system that mimics the human approach to image processing by following five key stages: Perception, Scheduling, Execution, Reflection, and Rescheduling. AgenticIR leverages large language models (LLMs) and vision-language models (VLMs) that interact via text generation to dynamically operate a toolbox of IR models. We fine-tune VLMs for image quality analysis and employ LLMs for reasoning, guiding the system step by step. To compensate for LLMs' lack of specific IR knowledge and experience, we introduce a self-exploration method, allowing the LLM to observe and summarize restoration results into referenceable documents. Experiments demonstrate AgenticIR's potential in handling complex IR tasks, representing a promising path toward achieving general intelligence in visual processing.

==> figs/consistency/main.tex <==
\hspace{-4mm}
\includegraphics[width=0.5\linewidth]{figs/consistency/entropy (bit).png}
\includegraphics[width=0.5\linewidth]{figs/consistency/variation ratio.png}

\vspace{-5pt}
\captionof{figure}{Comparison between dispersion of scheduling results with and without experience. Lower metric indicates higher consistency.\label{fig:cons}}

==> figs/main/main.tex <==
\begin{figure}[t]
    \scriptsize
    \centering
    \begin{minipage}[t]{0.3\linewidth}
    \vspace{-\fboxsep}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/0-input.png}
    \\
    Input image with rain and low resolution
    \end{minipage}
    % \hfill
    \hspace{1pt}
    \begin{minipage}[t]{0.6\linewidth}
    \vspace{-\fboxsep}
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/1-airnet.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/2-promptir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/3-mioir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/4-daclip.png}
    \end{minipage}
    \\
    \begin{minipage}{0.24\linewidth}
        \centering
        AirNet
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        PromptIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        MiOIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        DA-CLIP
    \end{minipage}  
    \\
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/5-instructir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/6-autodir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/7-random.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/A-rain+lr-6/8-ours(dr@res_sr@diff).png}
    \end{minipage}
    \\
    \begin{minipage}{0.24\linewidth}
        \centering
        InstructIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        AutoDIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        Random
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        \method
    \end{minipage}  
    \\
    \end{minipage}

    \vspace{-3pt}
    \begin{minipage}[t]{0.3\linewidth}
    \vspace{-\fboxsep}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/0-input.png}
    \\
    Input image low light, defocus blur, and JPEG compression artifact
    \end{minipage}
    % \hfill
    \hspace{1pt}
    \begin{minipage}[t]{0.6\linewidth}
    \vspace{-\fboxsep}
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/1-airnet.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/2-promptir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/3-mioir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/4-daclip.png}
    \end{minipage}
    \\
    \begin{minipage}{0.24\linewidth}
        \centering
        AirNet
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        PromptIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        MiOIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        DA-CLIP
    \end{minipage}  
    \\
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/5-instructir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/6-autodir.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/7-random.png}
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
    \includegraphics[width=\linewidth]{figs/main/C-dark+dfb+j-12/8-ours(dj@fbb_dfd@drb_br@g).png}
    \end{minipage}
    \\
    \begin{minipage}{0.24\linewidth}
        \centering
        InstructIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        AutoDIR
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        Random
    \end{minipage}
    \hfill
    \begin{minipage}{0.24\linewidth}
        \centering
        \method
    \end{minipage}  
    \\
    \end{minipage}
    \\
    \vspace{-10pt}
    \caption{Qualitative comparison with other methods.}
    \label{fig:main}
    \vspace{-10pt}
\end{figure}

==> figs/order/main.tex <==
\begin{figure}[t]
\scriptsize

\subfloat[{\fontsize{8pt}{\baselineskip}\selectfont Dehazing after denoising works but dehazing first fails.}\label{fig:order-hn}]{
\begin{minipage}{.485\linewidth}

\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/haze+noise/0-input.png}
Input image with haze and noise
\end{minipage}
%
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/haze+noise/1-denoise@restormer.png}
Result of denoising
\end{minipage}
% 
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/haze+noise/1-denoise@restormer_dehaze@xrestormer.png}
Result of first denoising and then dehazing
\end{minipage}


\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/haze+noise/HQ.png}
High-quality image
\end{minipage}
%
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/haze+noise/2-dehaze@xrestormer.png}
Result of dehazing
\end{minipage}
%
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/haze+noise/2-dehaze@xrestormer_denoise@restormer.png}
Result of first dehazing and then denoising
\end{minipage}
\vspace{-2pt}

\end{minipage}
}
% 
\hfill
% 
\subfloat[{\fontsize{8pt}{\baselineskip}\selectfont Deraining first works but deraining after SR fails.}\label{fig:order-rl}]{
\begin{minipage}{.485\linewidth}
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/rain+lr/0-input.png}
Input image with rain and low-resolution
\end{minipage}
%
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/rain+lr/1-derain@mprnet.png}
Result of deraining
\end{minipage}
%
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/rain+lr/1-derain@mprnet_sr@diffbir.png}
Result of first deraining and then SR
\end{minipage}


\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/rain+lr/HQ.png}
High-quality image
\end{minipage}
%
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/rain+lr/2-sr@diffbir.png}
Result of SR
\end{minipage}
% 
\hfill
% 
\begin{minipage}[t]{0.327\linewidth}
\includegraphics[width=\linewidth]{figs/order/rain+lr/2-sr@diffbir_derain@mprnet.png}
Result of first SR and then deraining
\end{minipage}

\vspace{-2pt}
\end{minipage}
}

\vspace{-7pt}
\caption{The importance of model selection and execution order in image restoration.\label{fig:order}}
\vspace{-6mm}
\end{figure}


==> figs/real/comparison.tex <==
\begin{figure}[t]
    \footnotesize
    \centering
    \includegraphics[width=0.19\linewidth]{figs/real/rainhaze/0-input.jpg}
    \hfill
    \includegraphics[width=0.19\linewidth]{figs/real/rainhaze/2-derain@restormer.jpg}
    \hfill
    \includegraphics[width=0.19\linewidth]{figs/real/rainhaze/3-dehaze@dehazefrmer.jpg}
    \hfill
    \includegraphics[width=0.19\linewidth]{figs/real/rainhaze/4-autodir_derain.jpg}
    \hfill
    \includegraphics[width=0.19\linewidth]{figs/real/rainhaze/1-derain@restormer-dehaze@dehazeformer.jpg}
    \\
    \begin{minipage}{.19\linewidth}
    \centering
    Input
    \end{minipage}
    \hfill
    \begin{minipage}{.19\linewidth}
    \centering
    Deraining by Restormer
    \end{minipage}
    \hfill
    \begin{minipage}{.19\linewidth}
    \centering
    Dehazing by Dehazeformer
    \end{minipage}
    \hfill
    \begin{minipage}{.19\linewidth}
    \centering
    AutoDIR
    \end{minipage}
    \hfill
    \begin{minipage}{.19\linewidth}
    \centering
    \method
    \end{minipage}
    \vspace{-6pt}
    \caption{Comparison with individual models on real-world images.}
    \label{fig:real-comp}
    \vspace{-10pt}
\end{figure}

==> figs/real/main.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.16\linewidth]{figs/real/udc/udc10_input_cropped.jpg}
    \hfill
    \includegraphics[width=0.16\linewidth]{figs/real/udc/udc10_output_cropped.jpg}
    \hfill
    \includegraphics[width=0.16\linewidth]{figs/real/underwater/9094_input_cropped.jpg}
    \hfill
    \includegraphics[width=0.16\linewidth]{figs/real/underwater/9094_output_cropped.jpg}
    \hfill
    \includegraphics[width=0.16\linewidth]{figs/real/rainhaze/0-input.jpg}
    \hfill
    \includegraphics[width=0.16\linewidth]{figs/real/rainhaze/1-derain@restormer-dehaze@dehazeformer.jpg}
    \vspace{-7pt}
    \caption{Examples of \method restoring real-world complexly degraded images. First two images: taken by under-display camera, restored by motion deblurring, defocus deblurring, and brightening; middle two images: taken underwater, restored by defocus deblurring, dehazing, and motion deblurring; last two: taken in heavy rain, restored by deraining and dehazing.}
    \label{fig:real}
    \vspace{-10pt}
\end{figure}

==> secs/1-intro_v0.tex <==
\section{Introduction}
Image restoration (IR) aims to reconstruct high-quality images from their low-quality counterparts, which are subject to various degradations like noise, blur, and haze.
%
Over the years, this field has witnessed lots of successful models dedicated to single-degradation restoration, \eg, denoising~\citep{DnCNN, MaskedDenoising}, deblurring~\citep{DeepDeblur, HI-Diff}, and dehazing~\citep{DCP, RIDCP}.
%
However, these models' effectiveness is only limited to a narrow range since their preoccupation is just some single specific degradation.

% However, in many real-world scenarios, we have no prior knowledge of the degradation type, and there may exist multiple degradations. Considering that we have lots of powerful single-degradation restoration tools, an intuitive way is to jointly utilize them to tackle such a complex-degradation restoration problem. 

Intuitively, if we collect multiple models for use, then the manageable input space will be the union of the models' respective input spaces. 
%
Furthermore, if we sequentially invoke multiple models, then the accessible output space will be much broader. This is a straightforward yet efficient way humans handle complex problems, treating the models as off-the-shelf tools.
%
Specifically, as for IR, multiple single-degradation restoration tools can be jointly utilized to address various kinds of degradations in the input image.
%
Such a complex-degradation restoration task~\citep{MPerceiver, InstructIR, AutoDIR, MiOIR, PromptGIP} is of both practical and academic value, as real-world images often suffer from multiple degradations, and entanglement among different degradations is worth research.

% Given several single-degradation restoration tools, to leverage them to realize complex-degradation restoration, 
To implement this,
%
several key points should be considered. 
%
First, we need to identify which tools to invoke; 
%
second, scheduling the order of tools often matters; 
%
besides, tools may fail unexpectedly. 
%
Overcoming these challenges requires flexible adaptability and rich knowledge of low-level vision.

In pursuit of such versatility, we resort to language agents, \ie, autonomous agents based on multi-modal large language models (MLLMs)~\citep{MSSurvey, FDSurvey, CoALA}. 
%
MLLMs acquire extensive general knowledge during pre-training on web-scale data and can thus rapidly transfer to new tasks~\citep{GPT4}. 
%
Many works equip MLLMs as ``brains'' with mechanism engineering~\citep{RUCSurvey} including tool usage~\citep{HuggingGPT, ControlLLM}, memory~\citep{GITM, GenerativeAgents}, exploration~\citep{Reflexion, AppAgent}, and planning~\citep{GITM, Self-Refine}, succeeding in various complex tasks.

In this paper, we construct a language agent that can automate the ensemble of single-degradation restoration tools to solve the challenging complex-degradation restoration task. 
%
To help the MLLM obtain expertise in low-level vision, we fine-tune it to inject the ability to recognize degradations, and let it self-explore to accumulate experience so as to make informed decisions when scheduling.
%
This learning paradigm fundamentally differs from previous approaches like symbolic rules or parameter optimization, featuring high efficiency and interpretability. 
%
We also bolster fault tolerance by iterative reflection.
%
This way, our agent could act just like a human expert, which resembles the long-sought-after artificial general intelligence in some aspect.
%
%
Our contribution can be summarized as follows:
\vspace{-5pt}
\begin{itemize}
    \item \textbf{Ensemble of IR tools:} To the best of our knowledge, we are the first to propose combining single-degradation restoration tools to tackle multiple unknown degradations.
    \item \textbf{IR result:} Our approach to complex-degradation restoration achieves decent performance comparable with existing all-in-one models~\citep{AirNet, TransWeather, PromptIR}, along with prominent efficiency and interpretability.
    \item \textbf{Language agent design:} We show how to enable MLLMs as generalists to complete professional tasks by novel learning paradigms, thus making a versatile language agent.
\end{itemize}
\vspace{-5pt}


==> secs/1-intro_v1.tex <==
\section{Introduction}
In the field of image restoration (IR), many models can successfully address degradation in images, preoccupied with specific tasks like denoising~\citep{DnCNN, MaskedDenoising}, deblurring~\citep{DeepDeblur, HI-Diff}, and dehazing~\citep{DCP, RIDCP}.
%
In this work, we propose an intelligent system that makes a combined usage of them to handle more general IR problems, treating the models as off-the-shelf tools.


The rationale behind this is straightforward:
%
if we collect multiple tools for use, then the manageable input space will be the union of the tools' respective input spaces;
%
furthermore, if we sequentially invoke multiple tools, then the accessible output space will be much broader.
%
This is an intuitive yet efficient way humans use tools at hand to handle complex problems.
%
For IR, multiple single-degradation restoration tools can be jointly utilized to address various kinds of degradations simultaneously present in the input image.
%
Such a complex-degradation restoration task is of both practical and academic value,
%
as real-world images may suffer from multiple degradations, and entanglement among different degradations is worth researching.
%


Solving this challenging task requires the system to possess high intelligence. 
%
Intelligence often entails perception and decision-making in an interactive environment. 
%
Here, perception is responsible for capturing relevant information from the environment, 
%
and careful decisions are accordingly made to exert effects on the environment, 
%
thus forming a loop.
%
The loop is necessitated by the complexity and uncertainty of the environment, \ie, it is hard to comprehensively predict the effects of decisions so as to make all decisions in one go.
%
An entity engaging in such a loop is commonly referred to as an \emph{agent}~\citep{agent-def, RL, FDSurvey}.
%

As for our agent system tasked with IR, perception focuses on the degradation of images, and decision-making is about which tool to invoke
%
(\eg, after recognizing noise and blur, whether to invoke the denoising tool or the deblurring tool).
%
Also, tools may fail unexpectedly since they are imperfect and the input images are complexly degraded.
%
This calls for reflection and retry in multiple interactions to ensure fault tolerance.
% %
% In view of the above considerations, we can conclude that our agent design should concentrate on the following aspects.
% %
% (1)~Perception: the agent can recognize various degradations in images. 
% %
% (2)~Decision-making: the agent can reliably decide the tool to invoke (\eg, after recognizing noise and blur, whether to invoke the denoising tool or the deblurring tool).
% %
% (3)~Interaction: an appropriate interaction paradigm can improve robustness.
%
Therefore, the situations faced are complex and diverse, demanding flexible adaptability and rich knowledge of low-level vision.

To obtain such versatility, we resort to multi-modal large language models (MLLMs), constructing a language agent~\citep{MSSurvey, FDSurvey, CoALA}. 
%
MLLMs acquire extensive general knowledge during pre-training on web-scale data and can thus rapidly transfer to new tasks~\citep{GPT4V}. 
%
Many works equip MLLMs as ``brains'' with mechanism engineering~\citep{RUCSurvey} including tool usage~\citep{HuggingGPT, ControlLLM}, memory~\citep{GITM, GenerativeAgents}, exploration~\citep{Reflexion, AppAgent}, and planning~\citep{GITM, Self-Refine}, succeeding in various complex tasks.

In this work, we construct a language agent that can automate the ensemble of single-degradation restoration tools to solve the complex-degradation restoration task. 
%
To help the MLLM acquire expertise in low-level vision, we fine-tune it to inject the ability to recognize degradations, and let it self-explore to accumulate experience to make informed decisions on scheduling.
%
This learning paradigm fundamentally differs from previous approaches like symbolic rules or parameter optimization, featuring high efficiency and interpretability. 
%
We also improve fault tolerance by iterative reflection.
%
This way, our agent could act just like a human expert, which resembles the long-sought-after artificial general intelligence in a sense.
%


==> secs/1-intro_v2.tex <==
\section{Introduction}
The image restoration community has contributed many models capable of addressing specific degradation in images like noise and haze.
%
Intuitively, combining multiple tools can greatly extend the range of manageable problems and accessible results.
%
Hence in real-world application scenarios, human users will comprehensively utilize various models to restore complexly degraded images, treating the models as off-the-shelf tools.
%
However, to our knowledge, at present there lacks a system automating this process.
%

To accomplish such a challenging goal, the system is supposed to possess adequate intelligence.
%
Intelligence often entails perception and action under a maintained plan in an interactive environment. 
%
Here, a plan is a sequence of actions to take.
%
After an action is taken, perception is responsible for capturing relevant information from the environment, and the plan is accordingly adjusted if needed.
%
This forms a loop.
%
The loop is necessitated by the complexity and uncertainty of the environment, \ie, it is hard to comprehensively predict the effects of actions to make all decisions in one go, so we need to maintain the plan online.
%
An entity engaging in such a loop is commonly referred to as an \emph{agent}~\citep{agent-def, RL, FDSurvey}.
%

As for our agent system tasked with image restoration, perception focuses on the degradation of images, and actions are invocations of image restoration tools.
%
The tools may fail unexpectedly since they are imperfect and the input images are complexly degraded.
%
This calls for reflection and retry in multiple interactions to ensure fault tolerance.
%
Therefore, the situations faced are complex and diverse, demanding flexible adaptability and rich knowledge of low-level vision.

To obtain such versatility, we resort to multi-modal large language models (MLLMs), constructing a language agent~\citep{MSSurvey, FDSurvey, CoALA}. 
%
MLLMs have extensive general knowledge and can thus rapidly transfer to new tasks~\citep{GPT4V}. 
%
Many works equip MLLMs as ``brains'' with mechanism engineering~\citep{RUCSurvey} including tool usage~\citep{HuggingGPT, ControlLLM}, memory~\citep{GITM, GenerativeAgents}, exploration~\citep{Reflexion, AppAgent}, and planning~\citep{GITM, Self-Refine}, succeeding in various complex tasks.


In this work, we construct a language agent that can automate the ensemble of single-degradation restoration tools to solve the complex-degradation restoration task 
%
(\ie, addressing multiple unknown degradations simultaneously present in the input image). 
%
The framework can be presented as tree search, enabling the agent to find a satisfactory result by deliberate thinking.
%
The search is guided by heuristics and pruning: confronted with an image with complex degradation, the appropriate tool is intelligently selected; after tool invocation, reflection is needed to determine whether to accept the result and go on.
%
This guidance comes from MLLMs directly, requiring expertise in low-level vision.
%
To qualify the MLLM for it, we fine-tune it to inject the ability to recognize degradations, and let it self-explore to accumulate experience so as to make informed decisions.
%
Such a learning paradigm fundamentally differs from previous approaches like symbolic rules or parameter optimization, featuring high efficiency and interpretability. 
%
This way, our agent system manifests as a neuro-symbolic architecture~\citep{LLMModulo}, acting just like a human expert and thus resembling the long-sought-after artificial general intelligence in a sense.
%


==> secs/1-intro_v3.tex <==
\section{Introduction}
The image restoration community has contributed many models capable of addressing specific degradation in images like noise and haze.
%
Intuitively, combining multiple tools can greatly extend the range of manageable problems and accessible results.
%
Hence in real-world application scenarios, human users will jointly utilize various models to restore complexly degraded images, treating the models as off-the-shelf tools.
%
However, completing this process involves some difficulties.
%
To name a few, how to select the tools to invoke? How to schedule the order of tools? What if a tool fails?
%
Overcoming these difficulties requires adequate \emph{intelligence}.


Intelligence often entails perception and action under a maintained plan in an interactive environment. 
%
Here, a plan is a sequence of actions to take.
%
After an action, perception is responsible for capturing relevant information from the environment, and the plan is accordingly adjusted if needed.
%
This forms a loop.
%
The loop is necessitated by the complexity and uncertainty of the environment, \ie, it is hard to comprehensively predict the effects of actions to make all decisions in one go, so we need to maintain the plan online~\citep{ReAct}.
%
An entity engaging in such a loop is commonly referred to as an \emph{agent}~\citep{agent-def, RL, FDSurvey}.
%


A principal problem is how the intelligent agent acquires the capability needed for a specific task.
%
In the simplest case, it is enough to just repeat practicing to memorize answers and then recall them in the face of similar problems, thanks to the lovely ergodic nature of the environment.
%
A more advanced paradigm advocates learning higher-level concepts:
%
as Plato’s allegory of the cave goes, there may exist unobservable laws that govern observed facts; 
%
once the latent laws are grasped, we can readily handle related tasks by applying them in combination with our prior knowledge including common sense and reasoning strategies.


As for our agent tasked with image restoration, perception focuses on the degradation of images, and actions are invocations of image restoration tools.
%
The tools may fail unexpectedly since they are imperfect and the input images are complexly degraded.
%
This calls for reflection and retry in multiple interactions to ensure fault tolerance.
%
Therefore, the situations faced are complex and diverse, demanding flexible adaptability and rich knowledge of low-level vision.

Large language models (LLMs) are rich in such versatility. 
%
They possess extensive general knowledge and can thus rapidly transfer to new tasks~\citep{GPT4}. 
%
Many works equip LLMs with mechanism engineering~\citep{RUCSurvey} including planning~\citep{ToT, RAP}, memory~\citep{GITM, GenerativeAgents}, tools~\citep{HuggingGPT, ControlLLM}, and exploration~\citep{Reflexion, AppAgent}, succeeding in various complex tasks.


In this work, we construct \method (Image Restoration Agent), an LLM-based agent that can automate the ensemble of single-degradation restoration tools to solve the complex-degradation restoration task 
%
(\ie, addressing multiple unknown degradations simultaneously present in the image). 
%
\cref{fig:framework} is an operational overview of \method.
%
The framework can be presented as tree search, enabling the agent to find a satisfactory result by deliberate thinking.
%
The search is guided by heuristics and pruning: confronted with an image with complex degradation, the appropriate tool is intelligently selected; following tool invocation, reflection is needed to determine whether to accept the result and go on.
%
Such guidance comes directly from LLMs, requiring expertise in low-level vision.
%
To qualify the LLM for it, we fine-tune it to inject the ability to recognize degradations, and let it self-explore to accumulate experience so as to make informed decisions.
%
Notably, a key decision is scheduling the order of single-degradation restoration subtasks, which is challenging even for human experts.
%
To tackle this problem, we prompt the agent to distill insights from accumulated experience, which are later retrieved to assist in scheduling.
%
Such a learning paradigm of exploring and verbally inferring latent laws fundamentally differs from previous approaches like symbolic rules or parameter optimization, featuring high efficiency and interpretability. 
%
This way, our agent system learns and infers to manipulate images just like humans and thus resembles the long-sought-after artificial general intelligence in a sense.
%

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/framework.pdf}
    \caption{An example illustrating the framework of our \method. (a) presents the entire workflow, where bubble frames beside robots represent responses from LLMs, and the numbers in circles correspond to those in (b). (b) points out the tree search nature of the system once the degradations are recognized. (c) expounds how to execute a single-degradation restoration subtask with a toolbox.}
    \label{fig:framework}
\end{figure}


==> secs/3-method_v0.tex <==
\section{Method}
Assume that for each type of degradation, a toolbox composed of several dedicated tools is available.
%
Our goal is to jointly utilize the toolboxes to restore an image with multiple unknown degradations.
%
\cref{sec:workflow} introduces our agent's workflow of restoring an image, and \cref{sec:ca} introduces how to equip the LLM, the brain of our agent, with the required expertise in low-level vision.


\begin{figure}[t]
\begin{minipage}{\linewidth}

\resizebox{0.4\linewidth}{!}{
\begin{minipage}{0.51\linewidth}
\footnotesize
\input{tables/pseudo_code}
\end{minipage}
}
\resizebox{0.6\linewidth}{!}{
\begin{minipage}{0.65\linewidth}
\input{figs/order/main}
\end{minipage}
}
\end{minipage}
\end{figure}


\subsection{Inference Workflow}
\label{sec:workflow} 
\paragraph{Entire workflow.}
\cref{fig:framework}a depicts an example of how our agent restores a complexly degraded image.
%
The agent first recognizes degradations in it to get the single-degradation restoration subtasks as an agenda.
%
The restored image will be the result of sequentially executing these subtasks, so the problem is reduced to finding the execution order.
%
Although the LLM can provide a suggestion (introduced later), there is no guarantee of its feasibility, hence reflection and adjustment are needed, calling for a more sophisticated search strategy.
%
This is a tree search problem as shown in \cref{fig:framework}b, each subtask being a node.
%
We design a depth-first search (DFS) control flow with heuristics and pruning.
%
Firstly, the agent proposes an initial plan and tries to execute it.
%
After executing each subtask, the result is checked;
%
if the subtask fails, the plan should be adjusted:
%
the agent rolls back this subtask execution and reschedules the order of subtasks in the current agenda.
%
If all possible execution orders fail, the agent rolls back further;
%
in case all orders from the root fail, the agent compromises to accept the best image yet and picks up the corresponding remaining plan.
%
\cref{alg:workflow} and \ref{alg:dfs} describe the process, where the functions except DFS are implemented by LLMs and detailed in \cref{supp:sec:llm}.


\paragraph{Subtask execution.}
For a single-degradation restoration subtask, the agent tries to execute it with access to several dedicated tools, as illustrated in \cref{fig:framework}c.
%
The agent randomly selects a tool, invokes it, and reflects on the tool result.
%
If satisfactory, then the tool result is output as the subtask result;
%
otherwise, the agent will reject it and continue to try other tools.
%
In case the tools are used up without passing the reflection, this subtask is reported as failed.
% 
For more details, refer to \cref{supp:sec:exe}.


\subsection{Capability Acquisition}
\label{sec:ca}
The agent should possess two critical capabilities: 
%
one is degradation evaluation, that is, given an image and a type of degradation, evaluating the severity of the degradation of the image; 
%
the other is subtasks scheduling, that is, given several single-restoration subtasks, scheduling their execution order.
%
Special strategies are needed to help the LLM, a powerful generalist, to learn such expertise.

\paragraph{Degradation evaluation.}
LLMs acquire extensive general knowledge during pre-training on web-scale data, which is a good starting point for learning domain knowledge.
% 
In view of this, we fine-tune a pre-trained LLM to inject the capability of degradation evaluation.
% 
The tuning data are question-answer pairs: given an image and a degradation, the question is ``What's the severity of \texttt{degradation} in this image?", and the answer is very low, low, medium, high, or very high.


\paragraph{Subtasks scheduling.}
The execution order of subtasks often greatly affects the restoration result, as exemplified by \cref{fig:order}.
% 
In \cref{fig:order-hn}, dehazing fails in the presence of noise, possibly because the high-frequency noise distorts the pattern of low-frequency haze;
% 
in \cref{fig:order-rl}, deraining fails after super-resolution, possibly because super-resolution distorts the pattern of rain.
% 
It can be seen that subtasks may have particular requirements and side effects,
% 
hence they should be carefully scheduled so that leading subtasks clear and do not introduce artifacts that distort requirements of following subtasks.
% 
Unfortunately, the LLM alone cannot do this.
% 
For example, in conversation 1 and 2 in \cref{tab:sche-bias}, we prompt GPT-4~\citep{GPT4}, the most powerful LLM so far, to schedule the order of motion deblurring and JPEG compression artifact removal.
% 
Strangely, when changing the presentation order of the two degradations, which is not relevant at all, the answer changes too:
% 
in conversation 1 it thinks removing compression artifacts will hinder deblurring, while in conversation 2 it thinks the opposite.
% 
We can see although having realized that subtasks have requirements and side effects, GPT-4 fails to address them reliably since it just imagines by itself.
% 
This echoes the argument from \cite{LLMModulo}: LLMs only have general planning knowledge but cannot deal with subtask interaction indeed, thus unable to give executable plans.
% 
Therefore, it is a must for the agent to get hands dirty, that is, exploring the actual situations to accumulate experience.
% 
For some complexly degraded images, we execute all possible subtask orders to comprehensively obtain restoration results, and then prompt the LLM to evaluate them.
% 
The evaluation statistics are concrete experience.
% 
Then we prompt the LLM to summarize them and distill insights, which serve as the agent's memory and are retrieved in inference to help subtasks scheduling.
% 
For example, when again prompting GPT-4 to schedule motion deblurring and JPEG compression artifact removal with the experience,
% 
it can find reference in the experience and thus consistently give an answer like response 3 in \cref{tab:sche-bias}.
% 
This way, GPT-4 can provide a reliable heuristic for the execution order of subtasks.


\begin{table}[t]
    \centering
    % \setlength\tabcolsep{3pt}
    \caption{Conversations with GPT-4~\citep{GPT4} to schedule subtasks.}
    \label{tab:sche-bias}
    \vspace{-8pt}
    \input{tables/schedule_bias}
\end{table}


==> secs/3-method_v1.tex <==
\section{Method}

Assume that for each type of degradation, a toolbox composed of several dedicated tools is available.
%
Our goal is to jointly utilize the toolboxes to restore an image with multiple unknown degradations.
%
\cref{sec:workflow} introduces our agent's workflow of restoring an image, and \cref{sec:ca} introduces how to equip the LLM, the brain of our agent, with the required expertise in low-level vision.


\begin{figure}[t]
\begin{minipage}{\linewidth}

\resizebox{0.4\linewidth}{!}{
\begin{minipage}{0.51\linewidth}
\footnotesize
\input{tables/pseudo_code}
\end{minipage}
}
\resizebox{0.6\linewidth}{!}{
\begin{minipage}{0.65\linewidth}
\input{figs/order/main}
\end{minipage}
}
\end{minipage}
\end{figure}


\subsection{Inference Workflow}
\label{sec:workflow} 
\paragraph{Entire workflow.}
\cref{fig:framework}a depicts an example of how our agent restores a complexly degraded image.
%
The agent first recognizes degradations in it to get the single-degradation restoration subtasks as an agenda.
%
The restored image will be the result of sequentially executing these subtasks, so the problem is reduced to finding the execution order.
%
Although the LLM can provide a suggestion (introduced later), there is no guarantee of its feasibility, hence reflection and adjustment are needed, calling for a more sophisticated search strategy.
%
This is a tree search problem as shown in \cref{fig:framework}b, each subtask being a node.
%
We design a depth-first search (DFS) control flow with heuristics and pruning.
%
Firstly, the agent proposes an initial plan and tries to execute it.
%
After executing each subtask, the result is checked;
%
if the subtask fails, the plan should be adjusted:
%
the agent rolls back this subtask execution and reschedules the order of subtasks in the current agenda.
%
If all possible execution orders fail, the agent rolls back further;
%
in case all orders from the root fail, the agent compromises to accept the best image yet and picks up the corresponding remaining plan.
%
\cref{alg:workflow} and \ref{alg:dfs} describe the process, where the functions except DFS are implemented by LLMs and detailed in \cref{supp:sec:llm}.


\paragraph{Subtask execution.}
For a single-degradation restoration subtask, the agent tries to execute it with access to several dedicated tools, as illustrated in \cref{fig:framework}c.
%
The agent randomly selects a tool, invokes it, and reflects on the tool result.
%
If satisfactory, then the tool result is output as the subtask result;
%
otherwise, the agent will reject it and continue to try other tools.
%
In case the tools are used up without passing the reflection, this subtask is reported as failed.
% 
For more details, refer to \cref{supp:sec:exe}.


\subsection{Capability Acquisition}
\label{sec:ca}
The agent should possess two critical capabilities: 
%
one is degradation evaluation, that is, given an image and a type of degradation, evaluating the severity of the degradation of the image; 
%
the other is subtasks scheduling, that is, given several single-restoration subtasks, scheduling their execution order.
%
Special strategies are needed to help the LLM, a powerful generalist, to learn such expertise.

\paragraph{Degradation evaluation.}
VLMs acquire extensive general knowledge during pre-training on web-scale data, which is a good starting point for learning domain knowledge.
% 
In view of this, we fine-tune a pre-trained VLM to inject the capability of degradation evaluation.
% 
The tuning data are question-answer pairs: given an image and a degradation, the question is ``What's the severity of \texttt{degradation} in this image?", and the answer is very low, low, medium, high, or very high.


\paragraph{Subtasks scheduling.}
The execution order of subtasks often greatly affects the restoration result, as exemplified by \cref{fig:order}.
% 
In \cref{fig:order-hn}, dehazing fails in the presence of noise, possibly because the high-frequency noise distorts the pattern of low-frequency haze;
% 
in \cref{fig:order-rl}, deraining fails after super-resolution, possibly because super-resolution distorts the pattern of rain.
% 
It can be seen that subtasks may have particular requirements and side effects,
% 
hence they should be carefully scheduled so that leading subtasks clear and do not introduce artifacts that distort requirements of following subtasks.
% 
Unfortunately, the LLM alone cannot do this.
% 
For example, in conversation 1 and 2 in \cref{tab:sche-bias}, we prompt GPT-4~\citep{GPT4} to schedule the order of motion deblurring and JPEG compression artifact removal.
% 
Strangely, when changing the presentation order of the two degradations, which is not relevant at all, the answer changes too:
% 
in conversation 1 it thinks removing compression artifacts will hinder deblurring, while in conversation 2 it thinks the opposite.
% 
We can see although having realized that subtasks have requirements and side effects, GPT-4 fails to address them reliably since it just imagines by itself.
% 
This echoes the argument from \cite{LLMModulo}: LLMs only have general planning knowledge but cannot deal with subtask interaction indeed, thus unable to give executable plans.
% 
Therefore, it is a must for the agent to get hands dirty, that is, exploring the actual situations to accumulate experience.
% 
For some complexly degraded images, we execute all possible subtask orders to comprehensively obtain restoration results, and then prompt the LLM to evaluate them.
% 
The evaluation statistics are concrete experience.
% 
Then we prompt the LLM to summarize them and distill insights, which serve as the agent's memory and are retrieved in inference to help subtasks scheduling.
% 
For example, when again prompting GPT-4 to schedule motion deblurring and JPEG compression artifact removal with the experience,
% 
it can find reference in the experience and thus consistently give an answer like response 3 in \cref{tab:sche-bias}.
% 
This way, GPT-4 can provide a reliable heuristic for the execution order of subtasks.


\begin{table}[t]
    \centering
    % \setlength\tabcolsep{3pt}
    \caption{Conversations with GPT-4~\citep{GPT4} to schedule subtasks.}
    \label{tab:sche-bias}
    \vspace{-8pt}
    \input{tables/schedule_bias}
\end{table}


==> secs/4-experiments_v0.tex <==
\section{Experiments}

\subsection{Implementation Details}
\paragraph{Settings.} 
We consider eight types of degradations: low resolution, noise, motion blur, defocus blur, rain, haze, JPEG compression artifact, and low light.
% 
For each of them, we collect three to six cutting-edge models as a toolbox.
% 
We design 16 combinations of two to three degradations and divide them into groups A, B, and C in the ratio of 2:1:1.
% 
Degradation combinations in group A and B consist of two degradations, while those in group C consist of three degradations.
% 
During exploration, the agent is exposed to group A.
% 
More details can be found in \cref{supp:sec:data} and \ref{supp:sec:tools}.


\paragraph{Data.} 
DIV2K~\citep{DIV2K} and Flickr2K~\citep{Flickr2K} datasets are used for fine-tuning on degradation evaluation.
% 
We randomly add two to four degradations on each image to obtain 15,000 complexly degraded images.
% 
For each of them, we iterate the seven degradations\footnote{
The degradation ``low resolution'' is excluded since we can directly recognize it by checking the resolution.
} to synthesize seven question-answer pairs.
% 
We use MiO100~\citep{MiOIR} dataset consisting of 100 high-quality images for exploration and testing.
% 
The 16 degradation combinations are respectively added to each image.
% 
For each combination in group A, we allocate 20 images for exploration (160 in total).
% 
The remaining 1,440 images are used for testing.


\paragraph{Learning degradation evaluation.} 
DepictQA~\citep{DepictQAv2, DepictQA} is a multi-modal LLM fine-tuned on image quality assessment.
% 
We further fine-tune it on degradation evaluation by LoRA technique~\citep{LoRA}.
% 
Learning rate 0.0005, weight decay 0.001, and Adam optimizer ($\beta_1=0.9, \beta_2=0.95$) are used.
% 
We fine-tune DepictQA for one epoch with batch size 64 on 4 NVIDIA Tesla V100 GPUs. 


\paragraph{Learning subtasks scheduling.} 
For each of the images allocated for exploration, we apply all possible sequences of corresponding tools and let the fine-tuned DepictQA evaluate restored images to check whether the restoration is successful.
% 
Then for each subtask order, we calculate the success rate.
% 
After collecting these statistics, we prompt GPT-4 to summarize and distill them, and then dump the results as a knowledge base, which will be a concrete ground for subtasks scheduling.


\subsection{Image Restoration Results}
We test \method on our testing set for the complex-degradation restoration task.
% 
To our knowledge, there is no open-source work for IR tool ensemble yet, so we design a simple baseline: 
% 
with the degradations known, randomly selecting one tool for each degradation and invoking them in random order.
% 
Six image quality assessment metrics are used for evaluation: three full-reference metrics PSNR, SSIM~\citep{SSIM}, LPIPS~\citep{LPIPS}, and three non-reference metrics MANIQA~\citep{MANIQA}, CLIP-IQA~\citep{CLIPIQA}, MUSIQ~\citep{MUSIQ}.
% 
\cref{tab:random} lists the quantitative comparison.
% 
Our agent outperforms the baseline in most metrics.


As for the IR performance, we compare \method with several all-in-one models\footnote{
% 
Since these models are not trained on all the eight degradations considered in this paper, we do not use the official weights but train the models under their default configurations. 
% 
The training set includes 27.6K images and covers the eight degradations.}:
% 
AirNet~\citep{AirNet}, TransWeather~\citep{TransWeather}, and PromptIR~\citep{PromptIR}.
% 
\cref{tab:all-in-one} lists the quantitative comparison.
% 
Our agent wins in most metrics including almost all non-reference metrics.
% 
Note that by this comparison we do not intend to argue the superiority of \method over all-in-one models.
% 
Instead, we hope to verify that combining single-degradation restoration IR tools can achieve comparable performance with all-in-one models, so this approach is feasible and meaningful.
% 
After all, the intrinsic purpose of our agent is not IR but IR tool ensemble.


Qualitative comparison with the baseline and all-in-one models is shown in \cref{fig:main}.
% 
We can see \method effectively addresses all degradations and yields visually pleasing results.
% 
In contrast, random invocations may fail to find the appropriate subtask order and tools, and all-in-one models may struggle to address all degradations due to their diverse and even conflicting characteristics.
% 


\begin{table}[t]
\begin{minipage}{0.485\linewidth}
\input{tables/baseline}
\end{minipage}
\hfill
\begin{minipage}{0.5\linewidth}
\input{tables/fixed}
\end{minipage}
\end{table}

\input{figs/main/main}

\begin{figure}[t]
\begin{minipage}{0.48\linewidth}
\vspace{3pt}
\input{figs/consistency/main}
\end{minipage}
\hfill
\begin{minipage}{0.47\linewidth}
\input{tables/finetune_res}
\end{minipage}
\end{figure}


\subsection{Learning Outcome}
In this section, we check the outcome of learning expertise in low-level vision.


\subsubsection{Degradation Evaluation}
For each image in the testing set, we prompt the fine-tuned DepictQA to evaluate the severity of each degradation.
% 
Treating degradation evaluation as binary classification (\ie, whether the image suffers from the degradation), we compute the precision, recall, and F1 score, as listed in \cref{tab:finetune-res}.
% 
Considering we do not bother to design special strategies and the fine-tuning only consumes modest computational resources (three hours on four V100 GPUs), the learning is fairly effective.

\subsubsection{Subtasks Scheduling} 
Informed of successful rates of each subtask order for each degradation combination in group A, GPT-4 tries to summarize them and distill insights.
% 
\cref{tab:sche-ex} shows snippets of the distilled insights and how they help subtasks scheduling.
% 
We can see that GPT-4 does conclude general rules that seem reasonable and apply them to infer the order of subtasks logically.
% 
The scheduling of ``deraining, super-resolution" and ``denoising, dehazing" also echo our discussion about \cref{fig:order} in \cref{sec:ca}.
% 
To quantitatively evaluate the correctness of the plans derived from experience, we let the agent act as the plan to restore images in the testing set.
% 
As the control group, we conduct an experiment wherein the agent does not act as the plans.
% 
\cref{tab:fixed} lists the results, which indicate the efficacy of subtasks scheduling learning.
% 
For more details, refer to \cref{supp:sec:learn} and \ref{supp:sec:sche-res}.


We also investigate the consistency improvement to justify the motivation introduced in \cref{sec:ca}:
% 
for a degradation combination, GPT-4 fails to consistently give a scheduling result, especially sensitive to the presentation order of degradations; providing experience should alleviate this problem.
% 
We prompt GPT-4 to schedule each combination 60 times with random presentation order, and then measure the dispersion of the results.
% 
Two metrics are adopted: (1) treating the results as a discrete distribution over all permutations of subtasks, entropy reflects the overall dispersion;
% 
(2) variation ratio is the proportion of samples that are not mode, straightforwardly reflecting confidence in the dominant result.
% 
\cref{fig:cons} compares the dispersion of scheduling results of the 16 degradation combinations with and without experience averaged in groups.
% 
The consistency improvement supports our claim.
% 
For more details, refer to \cref{supp:sec:sche-cons}.

\begin{figure}[t]
\begin{minipage}{0.5\linewidth}
\input{tables/all-in-one}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\scriptsize
\input{figs/ablation/reflection/main}
\end{minipage}
\end{figure}


\begin{figure}[t]
\begin{minipage}{0.48\linewidth}
\scriptsize
\input{figs/ablation/retrieval/main}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
\scriptsize
\input{figs/ablation/rollback/main}
\end{minipage}
\end{figure}


\begin{table}[t]
\begin{minipage}{\linewidth}
\begin{minipage}{0.41\linewidth}
\scriptsize
\vspace{-10pt}
\input{tables/schedule_ex}
\end{minipage}
\hfill
\begin{minipage}{0.57\linewidth}
\footnotesize
\input{tables/ablation/main}
\end{minipage}
\end{minipage}
\end{table}


\subsection{Ablation Study}
There are three modules to ablate: 
% 
retrieval, \ie, whether to reference the experience when scheduling subtasks;
% 
reflection, \ie, whether to check the tool results;
% 
rollback, \ie, whether to roll back failed subtasks.
% 
We compare the performances with and without the three modules respectively\footnote{
% 
Reflection is a prerequisite of rollback, so rollback is disabled when ablating reflection.
}, 
% 
and the quantitative results are listed in \cref{tab:ablation}.
% 
It can be seen that the absence of any module leads to a performance drop in more than half metrics.
% 
% It is a little strange that retrieval hurts the performance on group A, which directly contributes to the experience.
% 


Qualitative comparisons are shown in \cref{fig:ab-ref}, \cref{fig:ab-retr}, and \cref{fig:ab-rb}.
% 
In \cref{fig:ab-ref}, without reflection, although the subtask orders are the same, the agent fails to select the appropriate tool, resulting in remnant degradation (noise in line 1 and JPEG compression artifact in line 2).
% 
In \cref{fig:ab-retr}, without retrieval, the agent fails to come up with the appropriate subtask orders: 
% 
in line 1 defocus deblurring distorts compression artifact, and in line 2 dehazing fails in the presence of noise.
% 
In \cref{fig:ab-rb}, without rollback, the agent fails to correct the suboptimal subtask order suggested by retrieval:
% 
in line 1, although defocus deblurring before SR makes sense, the defocus blur in this case is slight enough to be addressed by SR tools\footnote{
% 
The training data of many SR models also include blur, as proposed by \cite{Real-ESRGAN}.
},
% 
but first conducting defocus deblurring over-smoothens the image;
% 
in line 2, the experience does not provide guidance for scheduling denoising and deraining, so the agent's plan fails without adjustment.
% 
These examples clearly demonstrate that the three modules are necessary in various scenarios, working together to enable the agent to find the proper subtask order and tools.



==> secs/5-discussion_v0.tex <==
\section{Discussion}
\paragraph{Conclusion.}
In this work, we formulate the IR tool ensemble problem and implement an agentic solution.
% 
The proposed system has a neuro-symbolic architecture that fuses neural networks' response into mature hard-coded problem-solving strategies~\citep{PolanyiRevenge}:
% 
the DFS-like control flow with reflection and rollback enables the agent to infer in a principled and efficient way,
% 
and LLMs can harness the potential of data.
% 
Besides, a novel learning paradigm is employed that prompts the agent to verbally learn from self-exploration.
% 
This work may lay a foundation for a purposed and skillful language agent specialized in low-level vision.

\paragraph{Limitation.}
Our primary goal is to realize an intelligent agent for IR tool ensemble, but this paper only considers single-degradation restoration tools, limiting the application to the so-called complex-degradation restoration problem.
% 
It is worth exploring whether our paradigm can integrate more general and heterogeneous tools,
% 
which will require higher flexibility and decision-making capabilities.
% 
A generally capable agent is supposed to surmount these challenges.


==> tables/ablation/main.tex <==
\begin{table}[t]
\caption{Ablation studies of the inference workflow, including reflection (Ref.) and rollback (Rb.).}
\label{tab:ablation}
\centering

\setlength\tabcolsep{1pt}

\vspace{-5pt}
\subfloat[Ablation study of reflection.\label{tab:ab-ref}]{
\resizebox{0.5\linewidth}{!}{
\input{tables/ablation/reflection}
}
}
\subfloat[Ablation study of rollback.\label{tab:ab-rb}]{
\resizebox{0.5\linewidth}{!}{
\input{tables/ablation/rollback}
}
}
\vspace{-8mm}
\end{table}


==> tables/all-in-one.tex <==
\begin{wraptable}{r}{0.6\linewidth}
\vspace{-10pt}
% \captionof{table}{Quantitative comparison with all-in-one models. The best and second best performances are marked in \best{bold} and \sbest{underline} respectively.\label{tab:all-in-one}}
\caption{Quantitative comparison with all-in-one models. The best and second best performances are marked in \best{bold} and \sbest{underline} respectively.\label{tab:all-in-one}}
\setlength\tabcolsep{2pt}
\centering
% \vspace{1pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\toprule
Degradations & Method &PSNR & SSIM & LPIPS$\downarrow$ & MANIQA & CLIP-IQA & MUSIQ\\
\midrule
 \multirow{7}{*}{Group A} 
  & AirNet & 19.13& 0.6019& 0.4283& 0.2581& 0.3930& 42.46\\
  & PromptIR & 20.06& 0.6088& 0.4127& 0.2633& 0.4013& 42.62\\
  & MiOIR & \sbest{20.84}& \sbest{0.6558}& \sbest{0.3715}& 0.2451& 0.3933& \sbest{47.82}\\
  & DA-CLIP & 19.58& 0.6032& 0.4266& 0.2418& \sbest{0.4139}& 42.51\\
  & InstructIR & 18.03& 0.5751& 0.4429& \sbest{0.2660}& 0.3528& 45.77\\
  & AutoDIR & 19.64& 0.6286& 0.3967& 0.2500& 0.3767& 47.01\\
  & \method & \best{21.04}& \best{0.6818}& \best{0.3148}& \best{0.3071}& \best{0.4474}& \best{56.88}\\
\midrule
 \multirow{7}{*}{Group B} 
  & AirNet & 19.31& 0.6567& 0.3670& 0.2882& 0.4274& 47.88\\
  & PromptIR & 20.47& 0.6704& 0.3370& 0.2893& 0.4289& 48.10\\
  & MiOIR & \best{20.56}& \sbest{0.6905}& \sbest{0.3243}& 0.2638& \sbest{0.4330}& \sbest{51.87}\\
  & DA-CLIP & 18.56& 0.5946& 0.4405& 0.2435& 0.4154& 43.70\\
  & InstructIR & 18.34& 0.6235& 0.4072& \sbest{0.3022}& 0.3790& 50.94\\
  & AutoDIR & 19.90& 0.6643& 0.3542& 0.2534& 0.3986& 49.64\\
  & \method & \sbest{20.55}& \best{0.7009}& \best{0.3072}& \best{0.3204}& \best{0.4648}& \best{57.57}\\
\midrule
 \multirow{7}{*}{Group C}
  & AirNet & 17.95& 0.5145& 0.5782& 0.1854& 0.3113& 30.12\\
  & PromptIR & 18.51& 0.5166& 0.5756& 0.1906& 0.3104& 29.71\\
  & MiOIR & 15.63& 0.4896& 0.5376& 0.1717& 0.2891& \sbest{37.95}\\
  & DA-CLIP & 18.53& 0.5320& 0.5335& 0.1916& \sbest{0.3476}& 33.87\\
  & InstructIR & 17.09& 0.5135& 0.5582& 0.1732& 0.2537& 33.69\\
  & AutoDIR & \sbest{18.61}& \sbest{0.5443}& \sbest{0.5019}& \sbest{0.2045}& 0.2939& 37.86\\
  & \method & \best{18.82}& \best{0.5474}& \best{0.4493}& \best{0.2698}& \best{0.3948}& \best{48.68}\\
\bottomrule
\end{tabular}
\vspace{-20pt}
}
\end{wraptable}


==> tables/finetune_res.tex <==
% \begin{table}[t]
% \begin{wraptable}{r}{0.5\linewidth}
% \caption{Degradation evaluation performance of fine-tuned DepictQA.}
\captionof{table}{Degradation evaluation performance of fine-tuned DepictQA.\label{tab:finetune-res}}
\centering
\setlength\tabcolsep{3pt}
\vspace{-5pt}
\resizebox{\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    Degradation               & Precision & Recall & F1 score  \\
    \midrule
    Noise                     & 0.99      & 0.92   & 0.95       \\
    Motion blur               & 0.88      & 0.52   & 0.65       \\
    Defocus blur              & 0.82      & 0.65   & 0.72       \\
    JPEG compression artifact & 0.98      & 1.00   & 0.99 \\
    Rain                      & 0.97      & 0.98   & 0.98       \\
    Haze                      & 0.88      & 0.91   & 0.89       \\
    Low light                      & 0.87      & 0.65   & 0.74       \\
    \bottomrule
    \end{tabular}
}
% \end{wraptable}

==> tables/fixed.tex <==
\captionof{table}{Quantitative comparison between acting as the agent's plan and the opposite. ``Not as planned" means randomly shuffling the plan (guaranteed to be different).\label{tab:fixed}}

\setlength\tabcolsep{2pt}
\vspace{-6pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\toprule
Degradations & As planned &PSNR & SSIM & LPIPS$\downarrow$ & MANIQA & CLIP-IQA & MUSIQ\\
\midrule
 \multirow{2}{*}{Group A} & \cmark & \best{21.14}& \best{0.6836}& \best{0.2753}& \best{0.3469}& \best{0.5091}& \best{60.77}\\
  & \xmark & 20.79& 0.6652& 0.3060& 0.3385& 0.4819& 59.85\\
\midrule
 \multirow{2}{*}{Group B} & \cmark & \best{21.14}& \best{0.7088}& \best{0.2683}& 0.3588& \best{0.5275}& \best{61.92}\\
  & \xmark & 20.32& 0.6811& 0.2976& \best{0.3623}& 0.5257& 60.15\\
\midrule
 \multirow{2}{*}{Group C} & \cmark & \best{18.78}& \best{0.5352}& \best{0.4239}& \best{0.3118}& \best{0.4876}& 51.08\\
  & \xmark & 18.49& 0.5277& 0.4345& 0.3058& 0.4719& \best{51.32}\\
\bottomrule
\end{tabular}
}


==> tables/random.tex <==
\captionof{table}{Quantitative comparison with the random tool invocation. The better performances are marked in \best{bold}. $\downarrow$ means the lower the better, and for others, the higher the better.\label{tab:random}}

\centering
\setlength\tabcolsep{2pt}
\vspace{-6pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\toprule
Degradations & Method &PSNR & SSIM & LPIPS$\downarrow$ & MANIQA & CLIP-IQA & MUSIQ\\
\midrule
 \multirow{2}{*}{Group A} & \method & \best{21.04}& \best{0.6818}& \best{0.3148}& \best{0.3071}& \best{0.4474}& \best{56.88}\\
  & Random & 20.90& 0.6642& 0.3368& 0.2963& 0.4394& 55.30\\
\midrule
 \multirow{2}{*}{Group B} & \method & \best{20.55}& \best{0.7009}& \best{0.3072}& \best{0.3204}& \best{0.4648}& \best{57.57}\\
  & Random & 20.06& 0.6766& 0.3351& 0.3120& 0.4514& 56.15\\
\midrule
 \multirow{2}{*}{Group C} & \method & 18.82& \best{0.5474}& \best{0.4493}& \best{0.2698}& \best{0.3948}& \best{48.68}\\
  & Random & \best{18.87}& 0.5456& 0.4796& 0.2354& 0.3543& 44.61\\
\bottomrule
\end{tabular}
}

==> tables/schedule_bias.tex <==
\begin{table}[t]
\centering
% \setlength\tabcolsep{3pt}
\caption{Prompting GPT-4~\citep{GPT4} to plan.}
\label{tab:sche-bias}
\vspace{-8pt}

\resizebox{\linewidth}{!}{
\begin{tabular}{cllc}
\toprule
ID & Prompt & Response &
\\ \midrule
1 &
\begin{minipage}{0.435\linewidth}
\scriptsize
\hytt{... we will conduct these tasks: \textcolor{red}{['motion deblurring', 'jpeg compression artifact removal']}. Please provide some insights into the correct order of these unordered tasks.}
\end{minipage} &
\begin{minipage}{0.435\linewidth}
\scriptsize
% \hytt{... JPEG compression artifacts can become more pronounced after other image processing tasks, such as sharpening or deblurring, because these tasks can accentuate the edges of the artifacts or introduce additional artifacts ...}
\hytt{... Motion deblurring should
ideally be performed first because it works best on images that have
not been subjected to additional processing ...}
\end{minipage}
&
\xmark
% \multirow{5}{*}{\xmark}
\\ \midrule
% \cline{1-3}
2 & 
\begin{minipage}{0.435\linewidth}
\scriptsize
\hytt{... we will conduct these tasks: \textcolor{red}{['jpeg compression artifact removal', 'motion deblurring']}. Please provide some insights into the correct order of these unordered tasks.}
\end{minipage} &
\begin{minipage}{0.435\linewidth}
\scriptsize
\hytt{... deblurring itself may exacerbate the appearance of compression artifacts, as it attempts to sharpen the image and restore detail ...}
\end{minipage} & \xmark
\\ \midrule
3 &
\begin{minipage}{0.435\linewidth}
\scriptsize
\hytt{... we will conduct these tasks: ['motion deblurring', 'jpeg compression artifact removal'] ... \textcolor{mydarkgreen}{we have the following experience} ... please give the correct order of the tasks.}
\end{minipage} &
\begin{minipage}{0.435\linewidth}
\scriptsize
\hytt{... \textcolor{mydarkgreen}{the experience suggests that} it is often better to remove artifacts before improving the image's content or quality ... we should remove JPEG artifacts before addressing the motion blur.}
\end{minipage} &
\cmark
\\ \bottomrule
\end{tabular}
}
\vspace{-7mm}
\end{table}


==> tables/schedule_ex.tex <==
% \captionof{table}{GPT-4's response for subtasks scheduling.\label{tab:sche-ex}}
\begin{table}[t]
\caption{GPT-4's response for subtasks scheduling.}
\label{tab:sche-ex}

\vspace{-5pt}

\setlength\tabcolsep{0.5mm}
\begin{tabular}{l}
\toprule
\begin{minipage}{\linewidth}
Insights distilled from experience
\end{minipage}
\\ \midrule
\begin{minipage}{\linewidth}
\scriptsize
\hytt{... better to remove artifacts (rain, JPEG compression) before improving the image's content or quality ...}
\end{minipage}
\\ \midrule
\begin{minipage}{\linewidth}
Scheduling deraining and super-resolution (in group A)
\end{minipage}
\\ \midrule
\begin{minipage}{\linewidth}
\scriptsize
\hytt{According to the collected experience, specifically point 8, it is more effective to address the artifact caused by rain before enhancing the image's resolution ...}
\end{minipage}
\\ \midrule
\begin{minipage}{\linewidth}
Scheduling denoising and dehazing (in group B)
\end{minipage}
\\ \midrule
\begin{minipage}{\linewidth}
\scriptsize
\hytt{... we can infer from the guidelines that issues related to image content enhancement should be addressed after dealing with artifacts. Since noise can be considered an artifact and dehazing is related to enhancing image content by removing haze, it would be logical to denoise the image before dehazing it.}
\end{minipage}
\\ \midrule
\begin{minipage}{\linewidth}
Scheduling brightening, defocus deblurring, and JPEG compression artifact removal (in group C)
\end{minipage}
\\ \midrule
\begin{minipage}{\linewidth}
\scriptsize
\hytt{... more effective to address blurring issues before image content enhancement ... removing artifacts like JPEG compression should be done before addressing blurring issues. Therefore, the order should start with JPEG compression artifact removal, followed by defocus deblurring, and finally brightening the image.}
\end{minipage}
\\ \bottomrule
\end{tabular}
\end{table}

